NAS-Bench-Suite: NAS Evaluation is (Now) Surprisingly Easy

The release of tabular benchmarks, such as NAS-Bench-101 and NAS-Bench-201, has significantly lowered the computational overhead for conducting scientific research in neural architecture search (NAS). Although they have been widely adopted and used to tune real-world NAS algorithms, these benchmarks are limited to small search spaces and focus solely on image classification. Recently, several new NAS benchmarks have been introduced that cover significantly larger search spaces over a wide range of tasks, including object detection, speech recognition, and natural language processing. However, substantial differences among these NAS benchmarks have so far prevented their widespread adoption, limiting researchers to using just a few benchmarks. In this work, we present an in-depth analysis of popular NAS algorithms and performance prediction methods across 25 different combinations of search spaces and datasets, finding that many conclusions drawn from a few NAS benchmarks do not generalize to other benchmarks. To help remedy this problem, we introduce NAS-Bench-Suite, a comprehensive and extensible collection of NAS benchmarks, accessible through a unified interface, created with the aim to facilitate reproducible, generalizable, and rapid NAS research. Our code is available at https://github.com/automl/naslib.

==> sections/11_nas_checklist.tex <==
\begin{comment}

\section{Reproducibility Statement}\label{app:nas_checklist}

% ICLR 2022: Authors are strongly encouraged to include a paragraph-long Reproducibility Statement at the end of the main text (before references) to discuss the efforts that have been made to ensure reproducibility. This paragraph should not itself describe details needed for reproducing the results, but rather reference the parts of the main paper, appendix, and supplemental materials that will help with reproducibility. 

For our reproducibility statement, we use the ``NAS Best Practices Checklist'' \citep{lindauer2019best}, which was recently released to improve reproducibility in neural architecture search.

%In the past, the field of NAS research has had problems with reproducibility and fairness in experimental comparisons~\citep{randomnas, nasbench, yang2019evaluation}. A NAS best practices checklist was recently released~\citep{lindauer2019best}, and we address each question below.

\end{comment}

%%%%% NOTE: often, including a reproducibility statement or submission checklist means we get auto-rejected from arxiv. But the NAS checkist is fine. So, I am changing the title and intro to this section. 


\section{NAS Research checklist}\label{app:nas_checklist}
There have been a few recent works which have called for improving the reproducibility and 
fairness in experimental comparisons in NAS research~\citep{randomnas, nasbench, yang2019evaluation}.
This led to the release of a NAS best practices checklist~\citep{lindauer2019best}.
We address each part of the checklist.



\begin{enumerate}

\item \textbf{Best Practices for Releasing Code}\\[0.2cm]
For all experiments you report: 
\begin{enumerate}
  \item Did you release code for the training pipeline used to evaluate the final architectures?
    \answerYes{Since we used NAS benchmarks for all of our experiments, we did not evaluate the
    architectures ourselves. The code for the training pipelines of these benchmarks is already
    publicly available.}
  \item Did you release code for the search space
    \answerYes{Again, since we used NAS benchmarks, this code is already
    publicly available.}
\item Did you release the hyperparameters used for the final evaluation pipeline, as well as random seeds?
  \answerYes{Since we used NAS benchmarks, the final training pipeline was fixed.
  We released our code, which includes the seeds used.}
  \item Did you release code for your NAS method?
  \answerYes{All of our code for benchmarking NAS methods is available at
  \url{https://github.com/automl/naslib}.}
  \item Did you release hyperparameters for your NAS method, as well as random seeds?
  \answerYes{The hyperparameters we used is also available at
  \url{https://github.com/automl/naslib}, and we discuss these choices in Appendix \ref{app:experiments}.}   
\end{enumerate}

\item \textbf{Best practices for comparing NAS methods}
\begin{enumerate}
  \item For all NAS methods you compare, did you use exactly the same NAS benchmark, including the same dataset (with the same training-test split), search space and code for training the architectures and hyperparameters for that code?
    \answerYes{We only used NAS benchmarks, which means the training details are 
    fixed.}
  \item Did you control for confounding factors (different hardware, versions of DL libraries, different runtimes for the different methods)?
    \answerYes{We only used NAS Benchmarks, which keep these details fixed.}	
    \item Did you run ablation studies?
    \answerNA{This is not applicable, because we did not devise a new NAS method.}
	\item Did you use the same evaluation protocol for the methods being compared?
    \answerYes{We only used NAS Benchmarks, which keep this fixed.}
	\item Did you compare performance over time?
    \answerNo{As we explained in Section \ref{sec:experiments}, since our focus was on comparing the relative performance across a large number of benchmarks, our plots focus on the performance across benchmarks while keeping runtime fixed for all methods.}
	\item Did you compare to random search?
    \answerYes{We did include random search in our experiments in Section \ref{sec:experiments}.}
	\item Did you perform multiple runs of your experiments and report seeds?
    \answerYes{We averaged 20 trials and 100 or more hyperparameter configurations for each experiment, and the choice of seeds (0-19) and hyperparameter configurations is available at \url{https://github.com/automl/naslib}.}
	\item Did you use tabular or surrogate benchmarks for in-depth evaluations?
    \answerYes{This is in fact one of the main purposes of our paper \smiley{}.}

\end{enumerate}

\item \textbf{Best practices for reporting important details}
\begin{enumerate}
  \item Did you report how you tuned hyperparameters, and what time and resources
this required?
    \answerYes{We reported this information in Section \ref{sec:experiments}.}
  \item Did you report the time for the entire end-to-end NAS method
    (rather than, e.g., only for the search phase)?
    \answerYes{Our results use the end-to-end time.}
  \item Did you report all the details of your experimental setup?
    \answerYes{We did include all details of the setup in Section \ref{sec:experiments} and \ref{app:experiments}.}

\end{enumerate}

\end{enumerate}

